Mind Your Weight(s): A Large-scale Study on Insufficient Machine Learning Model Protection in Mobile Apps

On-device machine learning (ML) is quickly gaining popularity among mobile apps. It allows offline model inference while preserving user privacy. However, ML models, considered as core intellectual properties of model owners, are now stored on billions of untrusted devices and subject to potential thefts. Leaked models can cause both severe financial loss and security consequences. This paper presents the first empirical study of ML model protection on mobile devices. Our study aims to answer three open questions with quantitative evidence: How widely is model protection used in apps? How robust are existing model protection techniques? What impacts can (stolen) models incur? To that end, we built a simple app analysis pipeline and analyzed 46,753 popular apps collected from the US and Chinese app markets. We identified 1,468 ML apps spanning all popular app categories. We found that, alarmingly, 41% of ML apps do not protect their models at all, which can be trivially stolen from app packages. Even for those apps that use model protection or encryption, we were able to extract the models from 66% of them via unsophisticated dynamic analysis techniques. The extracted models are mostly commercial products and used for face recognition, liveness detection, ID/bank card recognition, and malware detection. We quantitatively estimated the potential financial and security impact of a leaked model, which can amount to millions of dollars for different stakeholders. Our study reveals that on-device models are currently at high risk of being leaked; attackers are highly motivated to steal such models. Drawn from our large-scale study, we report our insights into this emerging security problem and discuss the technical challenges, hoping to inspire future research on robust and practical model protection for mobile devices.

==> Makefile <==
# Set this to one or more main LaTeX files (e.g. those with \documentclass) 
# for a specific build. Leave blank to build all files having an uncommented
# \documentclass.
MAIN=	


###########################################################################
#                 MAKE NO EDITS BELOW (except to debug)                   #
###########################################################################
#
#
# This is the PDFLATEX makefile, no support for ps/eps/dvi.
#
# Originally based on 
#   http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/Makefile
# but redeveloped by JG. Reuse by changing just the first line to list
# the main LaTeX source file.
#
# Features:
# - Finds all included LaTeX files, including includes within includes.
# - Finds all bibs and PDF figures included.
# - Automatically generates dependency information.
# - Repeats calls to PDFLATEX as necessary to fix cross references.
# - Displays missing references in a clean format at the end of the build.
# - Finds main LaTeX source files, so this makefile is reusable wihtout edits.
# - Works for files with bibliographies, and files without.

ifndef MAIN
MAIN:=	$(shell egrep -l "documentclass" *.tex)	
endif

ALLTEX:=$(shell ls *.tex)
ALLPDF:=$(ALLTEX:.tex=.pdf)

all pdf: $(MAIN:.tex=.pdf)
help ps dvi $(MAIN:.tex=.ps) $(MAIN:.tex=.dvi): die_unsupported
$(filter-out $(MAIN:.tex=.pdf),$(ALLPDF)): die_unsupported

%.pdf: %.fig
	rm -f $@
	fig2dev -L pdf $< > $@

%.aux: %.tex
	$(LATEX) $<

%.bbl: %.tex
	bibtex $(<:.tex=)
	$(LATEX) $<

%.pdf: %.aux
	@while (grep -q "Rerun to get" $(<:.aux=.log)) do \
		$(LATEX) $(<:.aux=.tex); \
	done
	@egrep -i "(Reference|Citation).*undefined" $(<:.aux=.log) ; true
	$(LATEX) $(<:.aux=.tex)

%.dep: %.tex
	@$(gettexs); $(getbibs); $(getfigs); \
	echo "$(<:.tex=.dep): Makefile " $$texs $$bibs $$figs > $@; \
	echo "$(<:.tex=.aux): " $$texs $$figs >> $@; \
	if [ $${#bibs} -gt 0 ]; then \
		echo "$(<:.tex=.bbl): " $$texs $$bibs >> $@; \
		echo "$(<:.tex=.pdf): $(<:.tex=.bbl)" >> $@; \
	fi

vpath %.fig figs

-include $(MAIN:.tex=.dep)

.PHONY: clean die_unsupported

double:
	for i in $(ALLTEX); do echo "Double words in $$i:" && ./double.pl < $$i; done

clean:
	rm -f *~ *.log *.aux *.dvi *.bbl *.blg *.cb *.dep $(TARGET)

copy:
	cp main.pdf ~/Desktop/modelxray.pdf

die_unsupported:
	$(warning Unsupported Makefile build target. Supported targets are:)
	$(warning  <BLANK> all pdf $(TARGET) clean)
	$(error Exiting)

LATEX=	pdflatex #--interaction batchmode
TARGET=	$(MAIN:.tex=.pdf)

# 9 Dec 2008 JG: This is now a worklist algorithm to pick up all recursive
#   child dependencies of discovered includes.
define gettexs
  worklist="$< "; \
  while [ $${#worklist} -gt 0 ]; do \
    curr=$${worklist%% *}; \
    worklist=$${worklist#* }; \
    texs="$${texs}$$curr "; \
    worklist=$${worklist}`perl -ne '\
               ($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/; \
	       @_=split /,/; \
	       foreach $$t (@_) { \
	         if ($$t !~ /\.tex$$/) { $$t .= ".tex"; } \
                 if (-e $$t) { print "$$t " } \
	       }' $${curr}`; \
	done
endef

define getbibs
  bibs=`perl -ne '\
        ($$_)=/^[^%]*\\\bibliography\{(.*?)\}/; \
        @_=split /,/; \
        foreach $$b (@_) { \
          if (-e "$$b.bib") { print "$$b.bib " } \
        }' $$texs`
endef

define getfigs
  figs=`perl -ne '\
        ($$_)=/^[^%]*\\\includegraphics(?:\[.*?\])?\{(.*?)\}/g; \
        if (defined($$_)) { \
          if ($$_ !~ /\.pdf$$/) { $$_ .= ".pdf"; } \
          if (-e $$_) { print "$$_ "; } \
        }' $$texs`
endef


==> evaluation.tex <==
\section{Evaluation}
In this section, we present the results from our app collection, static analysis, dynamic analysis and our financial loss model. 

\subsection{Apps using on-device ML}


In total, we were able to collect 46,753 Android apps from Google Play, Tencent My App and 360 Mobile Assistant stores. We integrated the app categories from these three stores, and sorted the top ten categories, as shows in Table \ref{tab:appinfo1}. It is interesting to see that the app distribution deviates from each store. For example, Google Play has more apps in Life category, and Tencent My App has equivalent number of apps in each category. While 360 Mobile Assistant intentionally makes every category having a number of 2,450 apps. 

On all these collected apps, we further applied our filtering criteria mentioned earlier in the static analysis, and found that 1,468 apps have ML models deployed on devices, which contributes to 3.14\% of the whole app collection. If we look into each store separately, the percentages of apps deploying on-device ML are 1.40\% for Google play, 7.25\% for Tencent My App and 3.55\% for 360 Mobile Assistant, meaning that in general Chinese app stores are more motivated in embracing ML in Android apps. There can be multiple reasons behind this percentage deviation, 
while one of the reasons can be the regulation differences regarding privacy concern. For example, ML models in business related apps may collect bank or ID card information that is considered as private, and health related apps may collect information that is considered as sensitive. 
% An evidence might be that, in Finance category, Google play has 4.88\% of the apps using ML while Tencent My App has 27.63\%. \textbf{(Not sure if this is a good example: 4.88\% is still higher than the general 1.40\%.)}
On the contrary, a beauty camera may just collect a photo that is less sensitive and most users would not hesitate to provide. Thus, when we look at the apps in Images category, the percentages of apps deploying ML become 10.32\% for Google play, 14.56\% for Tencent My App and 3.18\% for 360 Mobile Assistant---the percentage gap between US and Chinese app markets narrows. 


\begin{table}[!ht]
% \footnotesize
\centering
\caption{The number of apps collected across markets.}
\label{tab:appinfo1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{r|r|r|r|r|r|r|r|r}
\hline
 & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Google\\Play\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Tencent\\ My App\end{tabular}} & 
 \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}360\\ Mobile\\ Assistant\end{tabular}} &  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Total\end{tabular}} 
 \\ \hline
Category & All    & ML  & All   & ML & All   & ML  & All    & ML\\ \hline
Business & 404    & 2   & 99    & 2  & 2,450 & 296 & 2,953  & 300\\ 
News     & 96     & 0   & 102   & 5  & 2,450 & 180 & 2,648  & 185\\ 
Images   & 349    & 36  & 158   & 23 & 4,900 & 156 & 5,407  & 215\\ 
Map      & 263    & 4   & 206   & 14 & 2,450 & 83  & 2,919  & 101\\ 
Social   & 438    & 23  & 141   & 17 & 2,450 & 79  & 3,029  & 119\\ 
Shopping & 183    & 5   & 112   & 16 & 2,450 & 84  & 2,745  & 105\\ 
Life     & 1,715  & 15  & 193   & 16 & 2,450 & 53  & 4,358  & 84 \\
Education& 389    & 3   & 116   &  7 & 2,450 & 74  & 2,955  & 84 \\
Finance  & 123    & 6   & 76    & 21 & 2,450 & 55  & 2,649  & 82 \\
Health   & 317    & 5   & 115   & 3  & 2,450 & 42  & 2,882  & 50 \\
Other    & 8,434  & 79  & 874   & 35 & 4,900 & 29  & 14,208 & 143\\ \hline
\textbf{Total} 
         & 12,711 & 178 & 2,192 & 159& 31,850&1,131&46,753  &1,468\\ \hline
\end{tabular}
}
\footnotesize
{\raggedright \textit{Note}: In 360 Mobile Assistant store, the number of unique apps is 31,591 (smaller than 32,850) because some apps are multi-categorized, and the Images category contains 4,900 apps because we merged image and photo related apps.\par}
\end{table}


\noindent\textit{\textbf{\underline{$\bullet$ Insight}}: Including ML apps have the potential to increase the market share of an app store: Tencent My App has higher index than 360 Mobile Assistant \cite{appchina}, with fewer apps but higher percentage of ML apps. Developers interested in adding ML, if limited by regulations, may consider app stores worldwide.}

\subsection{ML functionalities and frameworks}
We further explored the functionalities of the ML models that the apps are using. The functionality of a ML model can be interpreted by the name of the library that invokes the ML model during runtime, according to the naming convention of most ML SDK providers \cite{Face++Services,Caffe2Framework.,TensorFlow}. 
The top ten widely used functionalities and the number of apps using them are showed in Table \ref{tab:store-ml-func}. 

Liveness detection models are the most widely used, as they are critical in detecting spoofing attacks, such as photos, masks and video images being used instead of the authorized person, to confuse the biometric recognition system \cite{Tan2010}. OCR, namely Optical Character Recognition, converts images of typed, handwritten or printed text into machine-encoded text, and is commonly used as a method of digitizing printed texts. Iris recognition uses the mathematical pattern of the images or videos of one or both of the irises of an individual's eyes as an automated method of biometric identification. In Google Play, OCR, face track, and face recognition are widely used, while ID card and bank card recognition functionalities are not found. In Tencent My App and 360 Mobile Assistant, the order of ML functionalities being used is almost the same, with widely adoption of ID card and bank card recognition.

\begin{table}[!ht]
\centering
% \footnotesize
\caption{The count of app using different ML functionalities.}
\label{tab:store-ml-func}
\resizebox{\columnwidth}{!}{% this table not as wide as the column
\begin{tabular}{r|r|r|r|r}
\hline
 Category & \begin{tabular}[c]{@{}c@{}}Google \\ Play\end{tabular} & \begin{tabular}[c]{@{}c@{}}Tencent \\ My App\end{tabular} & \begin{tabular}[c]{@{}c@{}}360 Mobile \\ Assistant\end{tabular} & Total \\ \hline
Liveness & 12 & 38 & 363 & 413 \\
ID card & 0 & 30 & 378 & 408 \\
OCR & 25 & 30 & 334 & 389 \\
Face track & 12 & 18 & 301 & 331 \\
Speech recognition& 7 & 14 & 213 & 234 \\
Bank card & 0 & 22 & 145 & 167 \\
Face recognition & 10 & 12 & 128 & 150 \\
Hand detect & 0 & 2 & 16 & 18 \\
Handwriting recognition & 2 & 3 & 5 & 10 \\
Iris recognition & 1 & 2 & 6 & 9 \\\hline
% \textcolor{red}{todo: Other} &  &  &  &  \\ \hline
% \textbf{Total} & 69 & 171 & 1,889 & 2,129 \\ \hline
\end{tabular}
}
\footnotesize
{\raggedright \textit{Note}: One app may use multiple ML functionalities, so the total number of apps is bigger than the total number of ML apps in Table \ref{tab:appinfo1}.\par}
\end{table}



% \subsection{ML frameworks}
Next, we show how these functionalities are distributed across different ML frameworks. Table \ref{tab:ml-frwk} presents the number of apps using some popular ML frameworks and their respective functionalities. As we can see, besides well known frameworks such as TensorFlow, TFLite, and Caffe, ML frameworks from the Chinese market such as SenseTime Parrots, Tencent NCNN \cite{Nihui}, and Xiaomi Mace \cite{ConvertingCode} are also widely used. Other frameworks, including MxNet from Apache \cite{ApacheLearning.} and ULS from Utility Asset Store \cite{UnityMaking} are also used many times in our app collection. 

Moreover, it is interesting to note that one app may use the same functionality from multiple frameworks. For example, a dictionary app {\tt com.youdao.hindict} uses both TensorFlow and Caffe in its OCR models. In fact, with some simple calculation, we found the case for one app using multiple frameworks is more common than we thought. Take Liveness as an example, the number of unique apps using it is 413 (Table \ref{tab:store-ml-func}), and adding up the number of apps from different ML frameworks is 1,281 (Table \ref{tab:ml-frwk}), therefore the average number of frameworks being used per app becomes 3.10 (1281$/$413). For handwriting recognition, this number increases to 6 (60$/$10). 

The reasons to use more than one frameworks per app are multifold. First, ML models can be conducted in different parts of an organization, and forcing work to be done in the same tools reduces efficiency and wastes resources. Second, integrating different frameworks allows engineers to choose the best functionality for pipelining, and ensures vendor flexibility. Finally, reusing an existing service or tool can prevent engineers from reinventing the wheels \cite{DataBlog}. 



\begin{table*}[!h]
\centering
% \footnotesize
\caption{Apps using different ML Frameworks with different functionalities.}
\label{tab:ml-frwk}
\resizebox{\textwidth}{!}{%
\begin{tabular}{r|r|r|r|r|r|r|r|r|r|r}
\hline
Category & \begin{tabular}[c]{@{}c@{}}TensorFlow \\ (Google)\end{tabular} & \begin{tabular}[c]{@{}c@{}}*Caffe2/PyTorch \\ (Facebook)\end{tabular} & \begin{tabular}[c]{@{}c@{}}*Parrots \\ (SenseTime)\end{tabular} & \begin{tabular}[c]{@{}c@{}}TFLite \\ (Google)\end{tabular} & \begin{tabular}[c]{@{}c@{}}NCNN \\ (Tencent)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mace \\ (Xiaomi)\end{tabular} & \begin{tabular}[c]{@{}c@{}}MxNet \\(Apache)\end{tabular} & \begin{tabular}[c]{@{}c@{}}ULS (Utility\\Asset Store)\end{tabular} & Other & Total \\
\hline
Liveness & 32 & 392 & 349 & 9 & 70 & 7 & 10 & 3 & 409 & 1,281 \\
ID card & 26 & 230 & 147 & 5 & 47 & 18 & 0 & 10 & 405 & 888 \\
OCR & 41 & 186 & 140 & 6 & 37 & 18 & 1 & 11 & 381 & 821 \\
Face track & 26 & 272 & 216 & 7 & 53 & 6 & 13 & 27 & 306 & 926 \\
Speech recognition& 7 & 32 & 9 & 1 & 11 & 18 & 1 & 9 & 230 & 318 \\
Bank card & 11 & 126 & 117 & 2 & 16 & 18 & 0 & 9 & 156 & 455 \\
Face recognition & 17 & 116 & 95 & 6 & 40 & 7 & 10 & 3 & 149 & 443 \\
Hand detect & 4 & 0 & 0 & 2 & 4 & 0 & 0 & 0 & 10 & 20 \\ 
Handwriting recognition & 8 & 17 & 1 & 0 & 16 & 0 & 0 & 0 & 18 & 60 \\
IRIS & 0 & 4 & 0 & 0 & 2 & 0 & 3 & 0 & 7 & 16 \\ \hline


\end{tabular}
}
\footnotesize
{\raggedright \textit{*} Caffe was initially open sourced by Berkeley. Then Facebook proposed Caffe2 by adding new features, and later merged Caffe2 to PyTorch. The following uses ``Caffe" to represent Caffe, Caffe2 and PyTorch. Parrots was not open sourced, and given that ``SenseTime" is used frequently in naming the models, the following use ``SenseTime" to represent both the framework and the company. \textit{Note}: 
One app may use multiple frameworks for one functionality, so the total number of apps is bigger than the total number of functionalities in Table \ref{tab:store-ml-func}.\par}
\end{table*}





\noindent\textit{\textbf{\underline{$\bullet$ Insight}}: Current model functionalities on mobile devices are straightforward and limited. Therefore, there is a great potential in including more diverse ML functionalities. Multi-framework is commonly adopted to reduce development cost. However, vulnerability in any framework may lead to whole functionality disrupted. We encourage companies to unify the ML framework in the long term.}

\subsection{Static Model Leakage}
Now that we have basic understanding of ML models in terms of Android markets, functionalities, and frameworks being used, the next step is to analyze how these models are protected in a statistical way. We aim to answer three questions: (1) Are apps designed to protect (e.g. encrypt) the ML models, or not? (2) If ML models are not protected, how severe is the problem? (3) Even if models are intentionally protected by the apps, are they really secure? The following will answer these questions from two perspectives: the app stores and the ML frameworks.

\subsubsection{Security across app stores}
Figure \ref{fig:model-security-store} gives an overview of app and model protection across three Android app stores. As Figure \ref{fig:app-enc} shows, in general, only 59\% of the apps are designed to protect their ML models. The rest of the apps include their models in plain text, and can be easily extracted after downloading their packages. We found 602 such apps in total, and these apps have been downloaded \textcolor{red}{xxx} times by the time this paper is written (Nov. 2019).

Additionally, when we look closer to each store, we found that Google Play has a lower protection rate at 26\%, while 360 Mobile Assistant and Tencent My App have rates at 59\% and 66\%, respectively. These rates indicate that Android apps from the Chinese markets are more motivated in protecting their ML models, either because of higher security awareness, or higher market demand \cite{Face++Services,SenseTime_1}.

Then, we calculated the number of models being protected in each store, as shows in Figure \ref{fig:model-enc}. The trend of model protection rates matches the observations of app protection rates in Figure \ref{fig:app-enc}, except with lower rate in each store. This can be explained by two facts. One fact is that some apps only protect their mission critical models, while leave the rest in plain text. However, this only represents a small portion of the whole collection. The other more important fact is that apps that do not protect the ML models are actually deploying more models than apps that do. 

\noindent\textit{\underline{\textbf{$\bullet$ Insight}}: Stealing models is easier than we thought, given the fact that some apps save the effort of protecting models to deploying more models. We show the consequence of model theft is critical, and we encourage app developers to spare more effort in model protection.}

As to the models being protected by the apps, we observed the same model being reused multiple times. For example, the most popular model {\tt SenseID\_Motion\_Liveness.model} has been used by 81 Android apps. What makes it even worse, this model is encrypted, and its MD5 hash appears in 81 apps. It means all these 81 apps are using the exactly same encryption and decryption key. Besides encryption key reuses among apps, a better case we observed is for one app reusing key among different versions, or among  releases across different app stores. This was found as we happened to collect the same app in different versions from Tencent My App and 360 Mobile Assistant.

\noindent\textit{\underline{\textbf{$\bullet$ Insight}}:
The reason for frequent model reuses can come from a ML SDK provider selling the same model to multiple companies. We believe that reusing the same key increases the risk of model leakage. The best practice should be changing the keys from app to app, and releases to releases. }


To see how severe is the reuse issue, we measured the reuse rate of all the models that are supposed to be protected by the apps across the three stores. As Figure \ref{fig:model-uniq} shows, in general, only 22\% of all the protected models are unique, meaning each model (with the same key) has been reused for 5 times, averagely. Among all stores, Google Play did a better job, with 80\% of unique models, while Tencent My App and 360 Mobile Assistant have unique rates of 50\% and 19\%, respectively. This can be explained that more apps are buying models from SDK providers in China than in US. Correspondingly, the risk for ML models to be leaked from Chinese app stores is higher than from Google Play.

\noindent\textit{\underline{\textbf{$\bullet$ Insight}}: Apps from Chinese markets tend to purchase ML models from SDK providers, because of the prosperous industry of AI solutions \cite{Face++Services,SenseTime_1,yitu}.
However, purchasing ML models transfer the responsibility of model protection from app developers to SDK providers. Given the high model reuse frequency, SDK providers have a long way to go. }

% Format of the figure carefully crafted, please don't change. Thanks!
\begin{figure*}[!h]
\centering
  \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[height=3.2cm]{figs/app-enc.png}
     \caption{App protection across stores.}
     \label{fig:app-enc}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[height=3.2cm]{figs/model-enc.png}
     \caption{Model protection across stores.}
     \label{fig:model-enc}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[height=3.2cm]{figs/model-uniq.png}
    \caption{Model reuse across stores.}
    \label{fig:model-uniq}
  \end{subfigure}
  \caption{Overview of app and model protection across different stores.}
  \label{fig:model-security-store}
\end{figure*}


% Format of the figure carefully crafted, please don't change. Thanks!
\begin{figure*}[!h]
\centering
  \begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\linewidth]{figs/app-fw-enc.png}
     \caption{App protection across frameworks.}
     \label{fig:app-fw-enc}
  \end{subfigure}
  \begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\linewidth]{figs/model-fw-enc.png}
     \caption{Model protection across frameworks.}
     \label{fig:model-fw-enc}
  \end{subfigure}
  \begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\linewidth]{figs/model-fw-uniq.png}
    \caption{Model reuse across frameworks.}
    \label{fig:model-fw-uniq}
  \end{subfigure}
  \caption{Overview of app and model protection across different frameworks. \textit{Note: MxNet, Mace, and ULS are merged into the 'Other' category due to their small numbers of apps and models involved.} }
  \label{fig:model-security-fw}

\end{figure*}


\subsubsection{Security across ML frameworks}
Now that we understand the distribution of model security problem across app stores, the next goal is to analyze the correlation between model protection and ML frameworks. As illustrated before, we calculated the app protection rate, model protection rate, and model reuse rate based on the whole app collection.

Figure \ref{fig:model-security-fw} shows the result in detail. MxNet, Mace, TFLite, and ULS are merged into the `Other’ category due to their small numbers of apps and models involved. For the rest of the ML frameworks, as shows in Figure \ref{fig:app-fw-enc}, more than 75\% of the apps protect the models when using SenseTime, and more than 50\% do it when using Caffe, while only around 20\% of the apps do it when using TensorFlow and NCNN.

As to the numbers of models, as shows in Figure \ref{fig:model-fw-enc}, the protection rate decreases for all frameworks. This matches with what we have observed in Figure \ref{fig:model-enc}---the unprotected apps are using more models than protected apps. It is interesting to note that 39\% of the models are protected when using Caffe, and this number beat SenseTime that has 24\% of the models protected, and TensorFlow and NCNN that both have 16\%. When we compare this result with Figure \ref{fig:model-uniq}, we observed similar trend as in Figure \ref{fig:model-uniq}---frameworks that have lower app and model protection rates, on the contrary, achieved higher percentage of model uniqueness, with TensorFlow and NCNN having around 40\% of the models being unique, while only 18\% of the models are unique when using SenseTime. 

% Since SenseTime enforces ML model encryption to its customers \cite{SenseTime_1}, we assume it has the awareness of the fact that model leakage can expose their customers to possible adversaries, and decrease its own market share among model SDK providers. Nevertheless, reusing the same model encryption key increases the potential of model leakage. Therefore, we suggest SenseTime to change its model encryption key from customers to customers.


\noindent\textit{\underline{\textbf{$\bullet$ Insight}}: Since SDK providers, e.g. SenseTime, enforce ML model encryption to their customers \cite{SenseTime_1}, we encourage them to check the results of this paper as a reference, and compare with their sale record to see whether their models have been leaked.}

\subsection{Dynamic Model Leakage}
Based on previous analysis, the most secure ML models by far are those protected and uniquely deployed in the Android apps. In this section, we focus on such models and try to extract them during app runtime. Since models need to be loaded into memory and being used in plain text, there is still chance to dump them from memory.

We started our manual analysis with the apps using most reused models, because of limited time. We were able to test 82 apps manually. The challenges of the tests come from several aspects. Some apps need registration, e.g. using a Chinese phone number, and authentication, e.g. linking a bank card, before triggering the ML function. While some apps have enabled too many functions for us to find the one that actually uses ML models in limited time. Some apps that we believe we have triggered its ML function, either load its ML model in the memory for a very short period of time, or in some unknown customized formats and contain no ML related keywords. 

Table \ref{tab:dump-model} demonstrates the results of our manual analysis. In total, we were able to dump the models from 18 apps out of 29 apps that we could trigger the ML functions. Given the fact that one of the apps contains two ML models that each has been reused for 81 times, we can then assume we are able to dump these two models from all the 81 apps. If we further assume we can dump the other ML models in these 81 apps, we basically are able to dump all the protected models from the whole collection. Even with a conservation estimation, given the average model reuse times of 4.5, and a percentage of 22\% (18 out of 82 apps) apps can be dumped, a semi-automated tool like the one used in this paper, can easily steal the ML models from 191 apps out of all the 866 apps with protected models, or 512 models out of the 2,321 protected models, and this could lead to \textcolor{red}{xxx} downloads of the apps/users involved. 

\noindent\textit{\textbf{\underline{$\bullet$ Insight}}: Model encryption makes it harder for attackers to steal models by simply decomposing the app package. Nevertheless, plain text of models still exist in memory during runtime, and a rooted phone can easy dump them. We therefore suggest developers to use customized formats for their model files, and strip/obfuscate ML-related keywords in strings. }

\begin{table}[!ht]
\caption{Overview of dumping models at runtime.}
\label{tab:dump-model}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{r|r|r|r|r} \hline
\multicolumn{1}{c|}{ML Framework} & \multicolumn{1}{c|}{Analyzed} & \multicolumn{1}{c|}{Extracted} & \multicolumn{1}{c|}{Cannot trigger} & \multicolumn{1}{c}{Cannot dump} \\ \hline
TensorFlow & 3 & 2 & 1 & 0 \\
Caffe & 7 & 1 & 4 & 2 \\
SenseTime & 55 & 11 & 39 & 5 \\
TFLite & 3 & 2 & 1 & 0 \\
NCNN & 9 & 0 & 6 & 3 \\
Other & 5 & 2 & 2 & 1 \\ \hline
\textbf{Total} & 82 & 18 & 53 & 11  \\ \hline
\end{tabular}
}
\end{table}


\begin{table*}[!ht]
\centering
\footnotesize
\caption{Overview of successfully dumped models and apps information from dynamic analysis.}
\label{tab:model-cases}
\begin{tabular}{l|l|l|l|l|l|l} \hline
App name                       & Model                         & Framework & Model function & Size (B) & Format & Reuses & Downloads & Extraction Method \\ \hline
com.basestonedata.instalment&  &  liveness_2.0_half.model      & TFLite    & Liveness Detection & 160K  & Flatbuffer & 18 & & Freed Buffer \\
sweetsnap.lite.snapchat        & faceprocessor.androidmodel    &Caffe      & Face Tracking         & 1.5M & Protobuf & 4 & ? & Model Loading \\
com.camera.one.s10.camera      & track\_face\_action1.0.0.model  & SenseTime & Face Tracking  & 2.3M & Protobuf & 77 & &Freed Buffer  \\
com.dailyselfie.newlook.studio & M\_SenseME_Action_5.5.1.model & SenseTime & Face Filter    & 3.6M & Protobuf & 3  & &Freed Buffer\\
video.like                     &M\_SenseME\_Face\_Extra\_5.22.0.model  & SenseTime  &Face Filter & 1.4M  & Protobuf  & 2 & & Freed Buffer \\
io.anyline.example.store       &USNr.any                               & Tensorflow & OCR  & 892K & Protobuf  &2 & & Memory Dumping  \\
com.baseapp.eyeem              &aesthetics-model.pb                    & Tensorflow & Photo Process & 6.5M & Protobuf &1 & & Freed Buffer  \\
com.decibel.beautycamera_101   &  &  &  &  &  &  \\
com.hepai.hepaiandroid &  &  &  &  &  &  \\
com.lemon.faceu &  &  &  &  &  &  \\
com.campmobile.snowcamera &  &  &  &  &  &  \\
sino.cargocome.carrier.droid &  &  &  &  &  &  \\
com.taojinjia.charlotte & SenseID\_Ocr\_Idcard_Mobile\_1.0.1.model & SenseTime  & OCR IDcard & 1.3M  & UnKnown & 13 &  & Freed Buffer  \\
com.kwai.video & unknown  & TFLite & Camera Filter & 228K & Json & 1 & & Freed Buffer \\
AntiVirus & optimized_graph.pb  & Tensorflow  & Malware Classification & 20M & 1 & & Decryption Method \\ \hline
\end{tabular}
\footnotesize
\\{\centering\textit{Note}: if needed.\par}
\end{table*}


% app name, framework, model function, size, format, reuse times, download times



